Enhancing 5G O-RAN Communication Efficiency Through AI-Based Latency Forecasting

The increasing complexity and dynamic nature of 5G open radio access networks (O-RAN) pose significant challenges to maintaining low latency, high throughput, and resource efficiency. While existing methods leverage machine learning for latency prediction and resource management, they often lack real-world scalability and hardware validation. This paper addresses these limitations by presenting an artificial intelligence-driven latency forecasting system integrated into a functional O-RAN prototype. The system uses a bidirectional long short-term memory model to predict latency in real time within a scalable, open-source framework built with FlexRIC. Experimental results demonstrate the model's efficacy, achieving a loss metric below 0.04, thus validating its applicability in dynamic 5G environments.

==> info <==
Recommendations for Improvement:
What It Is Missing:
Positioning Against State-of-the-Art:

While the related works section mentions other studies, the draft lacks a deeper critique of the gaps in those works, particularly in areas like "real-world hardware implementation" and "hyperparameter optimization" (Habib et al., Kavehmadavani et al.).
It should more explicitly identify the distinct contributions of the proposed approach, especially relative to the hardware and trade-off analyses.
Experimental Comparisons:

Many of the published papers include quantitative performance benchmarks against state-of-the-art systems. The draft paper's results section does not present comparative performance evaluations, which weakens its argument for novelty and superiority.
Scalability Testing:

Demonstrations of the system in varying traffic conditions or environments, as seen in similar studies (e.g., UAV-based mapping or 3D spectrum visualization), are absent. This leaves scalability claims unvalidated.
Reproducibility:

While reproducibility is highlighted, the paper lacks a clear description of datasets or specific experimental setups (e.g., configurations of srsRAN and Open5GS) necessary for reproducing results.
What Can Be Removed or Simplified:
Excessive Background Information:
The introduction spends too much time on explaining O-RAN challenges. Condensing this section can help focus on the novel aspects of the study.
Detailed Metric Lists:
Metrics such as "ues number," "rru prbtotul," and "snr" can be grouped or referenced in a supplementary table, simplifying the narrative.
Comparison with Other Papers:
Novelty: The draft attempts to combine forecasting with decision-making, which is unique compared to the predictive-only or analysis-centric focus of other papers. However, this should be more clearly articulated.
Clarity: Published works like "UAV-based CKM" and "RFID-ACCLDM" are better at explaining their methodologies step-by-step. The draft needs to emulate this clarity in presenting its experimental pipeline.
Validation: Most published works demonstrate their applicability through extensive scenarios or live demonstrations. The draft should include scenarios such as traffic spikes or hardware constraints for a more compelling case.
Alignment: The draft fits the conference's theme of practical systems (e.g., UAV-based and SLAM approaches). Its open-source, hardware-driven approach aligns well.
Actionable Steps:
Add comparative evaluations with at least one existing method (e.g., using simulation data for Habib et al. or real-time tests against Khalid et al.).
Revise and condense introductory sections to focus on unique contributions.
Expand experimental scenarios to include edge cases and scalability tests.
Enhance the related works discussion by explicitly stating gaps and how this work fills them.


%From the available KPMs in the Flexric, we have selected the following metrics to consider within the AI-based xApp to forecast the latency:
%\begin{itemize}
%    \item \textbf{ues\_number}: Tracks the number of User Equipment (UE) devices connected to the network. This metric aids in assessing network load and resource allocation.
%    \item \textbf{latency}: Measures the time delay experienced in the network, crucial for evaluating real-time performance and optimizing communication efficiency.
    %\item \textbf{rru\_prbavaildl}: Indicates the available physical resource blocks (PRBs) in the downlink for the Remote Radio Unit (RRU), reflecting the capacity left for new transmissions.
%    \item \textbf{rru\_prbavailul}: Indicates the available PRBs in the uplink for the RRU, monitoring resource availability for user data transmissions.
    %\item \textbf{rru\_prbtotdl}: Represents the total PRBs in the downlink, providing a benchmark for network capacity in that direction.
%    \item \textbf{rru\_prbtotul}: Represents the total PRBs in the uplink, serving as a baseline for uplink capacity.
%    \item \textbf{drb\_packetsuccessrateulgnbuu}: Monitors the packet success rate in the uplink at the gNB, showing transmission reliability.
    %\item \textbf{drb\_rlcpacketdropratedl}: Tracks the rate of packet drops in the downlink at the RLC layer, indicating possible inefficiencies or congestion.
   % \item \textbf{drb\_rlcsdutransmittedvolumedl}: Measures the volume of transmitted SDUs (Service Data Units) in the downlink via the RLC layer, representing data throughput.
%    \item \textbf{drb\_rlcsdutransmittedvolumeul}: Measures the SDUs transmitted in the uplink at the RLC layer, reflecting uplink throughput.
    %\item \textbf{drb\_uethpdl}: Tracks downlink throughput for UEs, giving insights into data delivery performance.
%    \item \textbf{drb\_uethpul}: Tracks uplink throughput for UEs, focusing on data transmission from UEs to the network.
%    \item \textbf{drb\_airifdelayul}: Monitors the air interface delay in the uplink, essential for understanding transmission latency over the air.
%    \item \textbf{snr}: The Signal-to-Noise Ratio, indicating the quality of the signal relative to background noise, influencing data rates and reliability.
%    \item \textbf{cqi}: The channel quality indicator, provided by the UEs, is used to adapt modulation and coding schemes to current channel conditions.
%    \item \textbf{timestamp}: Provides temporal alignment of collected data, enabling time-series analysis for trends and forecasting.
%\end{itemize}

As mentioned above, the system tracks several KPMs from Flexric to evaluate and optimize network performance. These include the number of connected UE devices to assess network load, latency for real-time performance evaluation, and uplink PRBs (available and total) to monitor resource availability and capacity. Metrics such as uplink packet success rate, transmitted SDUs, and throughput provide information on transmission reliability and efficiency, while air interface delay captures transmission latency. signal-to-noise ratio (SNR) and channel quality indicator (CQI) measure signal quality and channel conditions, enabling adaptive optimization. Finally, timestamps ensure temporal alignment for accurate time-series analysis and forecasting.

%Lastly, \textbf{timestamp} ensures temporal alignment of collected data, facilitating accurate time-series analysis and forecasting. Together, these KPMs offer a comprehensive view of network performance, enabling robust evaluation and dynamic optimization to meet operational goals.

As mentioned above, the system tracks several KPMs (Key Performance Metrics) from FlexRIC to evaluate and optimize network performance. These include the number of connected UE devices (\textbf{ues\_number}) to assess network load and resource allocation. Metrics such as \textbf{latency} measure the time delay experienced in the network, which is crucial for real-time performance evaluation and optimizing communication efficiency. 

Resource availability is monitored through \textbf{rru\_prbavailul} and \textbf{rru\_prbavaildl}, which indicate the available physical resource blocks (PRBs) in the uplink and downlink respectively, reflecting the capacity left for new transmissions. Similarly, \textbf{rru\_prbtotul} and \textbf{rru\_prbtotdl} represent the total PRBs in the uplink and downlink, providing a baseline for network capacity in both directions.

To assess transmission reliability and efficiency, the system tracks \textbf{drb\_packetsuccessrateulgnbuu}, which monitors the uplink packet success rate at the gNB. Metrics such as \textbf{drb\_rlcsdutransmittedvolumeul} and \textbf{drb\_rlcsdutransmittedvolumedl} measure the volume of transmitted SDUs (Service Data Units) in the uplink and downlink via the RLC layer, reflecting uplink and downlink throughput, respectively. Uplink and downlink throughput for UEs are further detailed by \textbf{drb\_uethpul} and \textbf{drb\_uethpdl}, offering insights into data delivery performance.

The air interface delay (\textbf{drb\_airifdelayul}) captures transmission latency over the air, while \textbf{snr} (Signal-to-Noise Ratio) and \textbf{cqi} (Channel Quality Indicator) provide measurements of signal quality and channel conditions. These are critical for enabling adaptive optimizations such as adjusting modulation and coding schemes. 
